Generalizable Local Feature Pre-training for Deformable Shape Analysis

Transfer learning is fundamental for addressing problems in settings with little training data. While several transfer learning approaches have been proposed in 3D, unfortunately, these solutions typically operate on an entire 3D object or even scene-level and thus, as we show, fail to generalize to new classes, such as deformable organic shapes. In addition, there is currently a lack of understanding of what makes pre-trained features transferable across significantly different 3D shape categories. In this paper, we make a step toward addressing these challenges. First, we analyze the link between feature locality and transferability in tasks involving deformable 3D objects, while also comparing different backbones and losses for local feature pre-training. We observe that with proper training, learned features can be useful in such tasks, but, crucially, only with an appropriate choice of the receptive field size. We then propose a differentiable method for optimizing the receptive field within 3D transfer learning. Jointly, this leads to the first learnable features that can successfully generalize to unseen classes of 3D shapes such as humans and animals. Our extensive experiments show that this approach leads to state-of-the-art results on several downstream tasks such as segmentation, shape correspondence, and classification. Our code is available at \url{https://github.com/pvnieo/vader}.

==> body/figure_animal_acc_evolution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/training_speed_animals.pdf}
    \caption{Evolution of the Mean Geodesic Error on the validation set, during the partial animal matching experiment. The dashed line in black shows that the performance, obtained by our features in the early stage of training, is still not reached by the competing features even after five times the training duration.}
    \label{fig:animals_evolution_acc}
\end{figure}

==> body/figure_cnn_filters.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/conv5_filters.png}
    \caption{Visualization for our feature extraction network. For each filter of the last 3D CNN layer (128 filters in total), we average the voxel grids ($16^{3}$) of top-100 training examples with the highest responses and extract surfaces from them using the marching cubes algorithm}
    \label{fig:cnn_filters}
\end{figure}


==> body/figure_pca.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unexplained_variance}
        \caption{Unexplained Variance}
        \label{fig:unexplained}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cross_unexplained_variance}
        \caption{Generalization Power}
        \label{fig:crossrec}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pca_projection.png}
        \caption{PCA Projection}
        \label{fig:embed_inclsion}
    \end{subfigure}
    \caption{PCA analysis of local patches from DFAUST and 3DMatch.}
    \label{fig:pretrain_data}
\end{figure}


==> body/figure_rna_acc_evolution.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/eval_acc_seg.pdf}
    \caption{Evolution of the RNA segmentation accuracy on the validation set, during the training of DiffusionNet with  different features.}
    \label{fig:rna_seg_evolution_acc}
\end{figure}



==> body/table_design_choice.tex <==
%\setlength{\tabcolsep}{4pt}
\begin{table}[!t]
    \begin{center}
        \resizebox{\columnwidth}{!}{%
            \begin{tabular}{lllrr}
                \hline
                \# & \textbf{Method} & \textbf{Dataset} & \textbf{FR on SR} & \textbf{SR on FR} \\
                \hline
                1. & FCGF            & ScanNet          & 20.4              & 9.1               \\
                2. & FCGF            & 3DMatch          & 19.3              & 19.6              \\
                3. & FCGF-L          & 3DMatch          & 4.8               & 7.9               \\
                4. & PCPNet-L        & 3DMatch          & 6.0               & 4.5               \\
                5. & 3DCNN-L         & DFAUST           & 27.7              & 4.4               \\
                6. & 3DCNN-L         & 3DMatch          & \textbf{4.1}      & \textbf{3.8}      \\
                \hline
            \end{tabular}
        }
        \caption{Results of using features pre-trained on different datasets and architectures on the downstream task of unsupervised non-rigid shape matching. ``-L'' denotes \textit{local} networks. Reported values are mean geodesic errors $\times 100$.}
        \label{tab:design_choice}
    \end{center}
\end{table}
%\setlength{\tabcolsep}{1.4pt}


==> body/table_sup_human_matching.tex <==
%\setlength{\tabcolsep}{4pt}
\begin{table}
    \begin{center}
        \begin{tabular}{lccc}
            \toprule
            \textbf{Method / Dataset}     & \textbf{FO}-\textbf{FR} & \textbf{FO}-\textbf{FQ} &
            \textbf{FO}-\textbf{SR}                                                                           \\
            \midrule
            MLP - XYZ                     & 13.8                    & 12.8                    & 26.9          \\
            MLP - HKS                     & 12.4                    & 21.5                    & 23.4          \\
            MLP - WKS                     & 12.7                     & 34.0                    & 27.2          \\
            MLP - SHOT                    & 10.0                    & 17.6                    & 10.6          \\
            MLP - PCH                     & 17.7                    & 41.5                    & 32.8          \\
            MLP - PCN                     & 15.7                    & 41.4                    & 28.4          \\
            MLP - \OurMethodName{} (ours) & \textbf{4.2}            & \textbf{4.9}            & \textbf{9.4} \\
            \bottomrule
        \end{tabular}
        \caption{Accuracy of various features for supervised shape matching when the connectivity changes from train to test.  X-Y means train on X and test on Y. Values are mean geodesic error $\times 100$ on unit-area shapes. \rev{Are the \OurMethodName{} results in this table up-to-date? If not, please remove the table. Corresponding discussions have been commented out.}}
        \label{tab:robust_connectivity}
    \end{center}
\end{table}
%\setlength{\tabcolsep}{1.4pt}

